Near-Linear Time Approximation Schemes for Clustering in Doubling Metrics

We consider the classic Facility Location, $k$-Median, and $k$-Means problems in metric spaces of doubling dimension $d$. We give nearly linear-time approximation schemes for each problem. The complexity of our algorithms is $2^{(\log(1/\eps)/\eps)^{O(d^2)}} n \log^4 n + 2^{O(d)} n \log^9 n$, making a significant improvement over the state-of-the-art algorithms which run in time $n^{(d/\eps)^{O(d)}}$. Moreover, we show how to extend the techniques used to get the first efficient approximation schemes for the problems of prize-collecting $k$-Medians and $k$-Means, and efficient bicriteria approximation schemes for $k$-Medians with outliers, $k$-Means with outliers and $k$-Center.

==> preamble.tex <==
\makeatletter
%\usepackage[sort,comma,square,numbers]{natbib}
%\renewcommand*{\NAT@spacechar}{~} %don't let citations make a line break
%\renewcommand\bibsection %don't introduce pagebreak for bibliography
%{
%  \section*{\refname
%    \@mkboth{\MakeUppercase{\refname}}{\MakeUppercase{\refname}}}
%}

% \usepackage{dsfont}             %
\usepackage[cmex10]{amsmath}
\interdisplaylinepenalty=2500

\usepackage{amsthm}
\usepackage{amssymb}
%\usepackage{algorithmicx}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{color}

\usepackage{comment}
%\usepackage{url}
\usepackage{hyperref}
\usepackage{xcolor}
\usepackage{subcaption}
\definecolor{darkblue}{rgb}{0,0,0.45}
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{darkgreen}{rgb}{0.13,0.5,0}
\hypersetup{colorlinks, linkcolor=darkblue, citecolor=darkgreen,
urlcolor=darkblue}

\usepackage{wrapfig}

\usepackage{authblk}

\usepackage[nameinlink,capitalise]{cleveref}
% \usepackage{mathabx}
%\usepackage[letterpaper,margin=1in]{geometry}
% 
%% \usepackage[moderate,lists=tight,mathdisplays=normal,mathspacing=normal,
%% wordspacing=normal,tracking=normal]{savetrees}

\usepackage{enumerate}
\usepackage{xcolor}

\newcommand{\set}[1]{\{#1\}}
\newcommand{\nbportals}{(\log n/\eps^{13})}
\renewcommand{\setminus}{-}
%% \newcommand{\calD}{\mathcal{D}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\I}{\mathcal{I}}
\newcommand{\ID}{\mathcal{I}_{\calD}}

% unbreakable hyphen:
\newcommand{\hy}{\hbox{-}\nobreak\hskip0pt}

\newcommand{\growthrate}{2}
\newcommand{\badcut}{\kappa(\eps, p)}
\newcommand{\offset}{\tau(\eps, d)}
\theoremstyle{plain}% default
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
% \newtheorem{defn}{Definition}[theorem]
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{claim}[theorem]{Claim}

% \theoremstyle{definition}
% \newtheorem{defn}{Definition}[theorem]
% \newtheorem{conj}{Conjecture}[theorem]
% \newtheorem{exmp}{Example}[theorem]
\theoremstyle{remark}
\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}
\newtheorem{case}{Case}

\newcommand{\capac}{h}

\newcommand{\tileta}{\tilde{h}}
\newcommand{\tid}{\tilde{d}}

\newcommand{\hF}{\hat{F}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\hL}{\hat{L}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tA}{\tilde{A}}

\newcommand{\hw}{h}
\newcommand{\chopt}{\text{charge}_{\globalS}}
\newcommand{\chol}{\text{charge}_{\local}}

\newcommand{\eps}{\varepsilon}
\newcommand{\opt}{\textup{OPT}}
\newcommand{\vor}{\text{Vor}}
\newcommand{\dist}{\textup{dist}}
\newcommand{\diam}{\textup{diam}}
\newcommand{\length}{\textup{length}}

\newcommand{\notetoself}[1]{\textbf{#1}}
\newcommand{\bigO}{O}
\newcommand{\cut}{\text{cut}}
\newcommand{\cact}{(g(k),f(k))\text{-cactus}}
\newcommand{\sep}{\text{sep}}
\newcommand{\del}{\text{Deletion}}
\newcommand{\bigS}{\mathcal{S}}
\newcommand{\cost}{\textup{cost}}
\newcommand{\Sercost}{\text{ServiceCost}}
\newcommand{\out}{\text{out}}
\newcommand{\ins}{\text{in}}
\newcommand{\event}{\mathcal{E}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\tcalV}{\tilde{\mathcal{V}}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\inter}{\text{int}}
\newcommand{\exter}{\text{ext}}
\newcommand{\spa}{\text{span}}
\newcommand{\local}{L}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\globalS}{\opt} % {\mathcal{G}}
\newcommand{\globalSs}{\opt^*} %{\mathcal{G}^{*}}
\newcommand{\Vloc}{V_{L}}
\newcommand{\Vglob}{V_{\opt}}
\newcommand{\globtoloc}{A_\local}
\newcommand{\loctoglob}{A_{\globalS}}
\newcommand{\reass}{\text{Reassign}}
%\newcommand{\globtoloc}{\text{Reassign}_{\globalSs \mapsto \local}}
%\newcommand{\loctoglob}{\text{Reassign}_{\local \mapsto \globalSs}}
\newcommand{\linelamb}{\overline{\Lambda_{\calR}^2}}
\newcommand{\costPeps}{(1+\eps_1)^p}
\newcommand{\costPepsn}{(1-\eps_1)^p}
\newcommand{\costPinv}{\eps_1^{-p}}
\newcommand{\spc}{\textsc{spc}}

\newcommand{\param}{100}
\newcommand{\tS}{\tilde{S}}
\newcommand{\regionsize}{O(d)}
\newcommand{\improv}{\text{Improv}}

\newcommand{\portalresp}{\text{moat-respecting}}
\newcommand{\netresp}{\text{moat-respecting}}
\newcommand{\irr}{\text{moat}}
\newcommand{\mirr}{\text{moat}}
\newcommand{\poly}{\text{poly}}

% \newcommand{\pr}{\mathbb{P}}

\newcommand{\wopt}{\widetilde{\opt}}

\newcommand{\epsval}{\eps}
\newcommand{\tc}{\tilde{c}}

\newcommand\E[1]{\mathbb{E}\left[\,#1\,\right]}

\def\imin{{i_{min}}}
\def\imax{{i_{max}}}
\def\imed{{i_{med}}}

\def\eg{\textit{e.g., }}
\def\ie{\textit{i.e., }}

\DeclareMathOperator*{\argmin}{arg\,min}

\def\note#1{\GenericWarning{}%
  {AUTHOR WARNING: Unresolved annotation}%
  {\marginpar%
    [\hfill\llap{\textcircled{\small{$\circledcirc$}}$\!\Longrightarrow$}]%
    {\rlap{$\Longleftarrow\!$\textcircled{\small{$\circledcirc$}}}}}%
  \textsf{$\langle\!\langle${\color{blue}{#1}}$\rangle\!\rangle$}%
}


% \newifshort
% \shorttrue % short version
%  \shortfalse % long version
\newcommand{\blue}[1]{{\color{blue}\bf #1}}
\newcommand{\gray}[1]{{\color{gray}\bf #1}}
\newcommand{\red}[1]{{\color{red}\bf #1}}
\newcommand{\magenta}[1]{{\color{magenta}\bf #1}}
\newcommand{\green}[1]{{\color{green}\bf #1}}
\newcounter{sideremark}
\newcommand{\marrow}{\stepcounter{sideremark}\marginpar{$\boldsymbol{
\longleftarrow\scriptstyle\arabic{sideremark}}$}}
\usepackage{setspace}
\newcommand{\paren}[1]{\left({#1}\right)}
\setlength{\marginparwidth}{1.4cm}
\newcommand{\marginnote}[3]{%\ifdraft 
$^{\textcolor{#2}{\mathbf{\dagger}}}$\marginpar{\setstretch{0.43}\textcolor{#2}{
\bf\tiny#1: #3}} %\fi
}

 \newcommand{\vincent}[1]{
 %  \ifdraft{
    \textsf{\magenta{*** (Vincent) \marrow #1 ***}}
 %  }
 %  \fi
 }
 
 \newcommand{\aef}[1]{
 %  \ifdraft{
  \textsf{\green{*** (Andreas) \marrow #1 ***}}
 %  }
 %  \fi
 }
 
 
 \newcommand{\david}[1]{
 %  \ifdraft{
    \textsf{\blue{*** (David) \marrow #1 ***}}
 %  }
 %  \fi
 }

\newtheoremstyle{rstate}%
{}{}%
{\itshape}{}%
{\bfseries}{}%  % Note that final punctuation is omitted.
{ }{}

\theoremstyle{rstate}
\newtheorem*{restate}{Theorem}

\makeatother

